Two-Stage Estimation and Variance Modeling for Latency-Constrained Variational Quantum Algorithms

The Quantum Approximate Optimization Algorithm (QAOA) has enjoyed increasing attention in noisy intermediate-scale quantum computing due to its application to combinatorial optimization problems. Because combinatorial optimization problems are NP-hard, QAOA could serve as a potential demonstration of quantum advantage in the future. As a hybrid quantum-classical algorithm, the classical component of QAOA resembles a simulation optimization problem, in which the simulation outcomes are attainable only through the quantum computer. The simulation that derives from QAOA exhibits two unique features that can have a substantial impact on the optimization process: (i) the variance of the stochastic objective values typically decreases in proportion to the optimality gap, and (ii) querying samples from a quantum computer introduces an additional latency overhead. In this paper, we introduce a novel stochastic trust-region method, derived from a derivative-free adaptive sampling trust-region optimization (ASTRO-DF) method, intended to efficiently solve the classical optimization problem in QAOA, by explicitly taking into account the two mentioned characteristics. The key idea behind the proposed algorithm involves constructing two separate local models in each iteration: a model of the objective function, and a model of the variance of the objective function. Exploiting the variance model allows us to both restrict the number of communications with the quantum computer, and also helps navigate the nonconvex objective landscapes typical in the QAOA optimization problems. We numerically demonstrate the superiority of our proposed algorithm using the SimOpt library and Qiskit, when we consider a metric of computational burden that explicitly accounts for communication costs.

==> mycommands.tex <==

%%% EDITING SHORTCUTS -----------------------------------------------------------------------------

\newcommand{\sara}[1]{{\color{red}{\textbf{[SS: #1]}}\color{black}}}
\newcommand{\saraedit}[1]{{\color{red}{#1}\color{red}}}

\newcommand{\stopped}{ \[=======================================================\]}
\newcommand{\done}{We agree. Done, thank you.}
\newcommand{\yunsoo}[1]{{\color{blue}{\textbf{[HA: #1]}}\color{black}}}
\newcommand{\annot}[1]{{\text{\normalfont #1}}}

%%% TEACHING SHORTCUTS -----------------------------------------------------------------------------

\newcommand{\answerblank}[1]{\underline{\makebox[#1][l]{ }}}

%%% MATH SHORTCUTS -----------------------------------------------------------------------------

% BEGIN: THIS CODE DEFINES THE \widebar COMMAND, WITH ADJUSTMENTS 

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother
% END: THIS CODE DEFINES THE \widebar COMMAND, WITH ADJUSTMENTS 


%argmin and argmax
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}

%real numbers
\newcommand{\real}{{\rm{I\hspace{-.75mm}R}}}
\newcommand{\ereal}{\widebar{\real}}

%operations
\newcommand{\domeq}{\preceq} %dominates, for multi-obj. work
\newcommand{\dom}{\prec}
\newcommand{\ndom}{\nprec}
\newcommand{\indic}[1]{\mathbb I\{#1\}}


%sums and products
\newcommand{\sumin}{\sum_{i=1}^n}
\newcommand{\sumir}{\sum_{i=1}^r}
\newcommand{\smsum}{\mathop{\textstyle\sum}}
\newcommand{\smsumin}{\mathop{\textstyle\sum}_{i=1}^n}
\newcommand{\smsumir}{\mathop{\textstyle\sum}_{i=1}^r}
\newcommand{\smprod}{\mathop{\textstyle\prod}}
\newcommand{\prodin}{\prod_{i=1}^n}

%fractions
\newcommand{\oon}{\frac{1}{n}} 
\newcommand{\oom}{\frac{1}{m}}
\newcommand{\oot}{\frac{1}{t}}
\newcommand{\oo}[1]{\frac{1}{#1}}
\newcommand{\ootwo}{\frac{1}{2}}
%\newcommand{\onehalf}[1]{\frac{#1}{2}}

\newcommand{\sqrtn}{\sqrt{n}}

%limits
\newcommand{\limn}{\lim_{n\rightarrow\infty}}
\newcommand{\limt}{\lim_{t\rightarrow\infty}}
\newcommand{\limnstack}{\displaystyle\lim_{n\rightarrow\infty}\textstyle}

%Statistical quantities and expressions
\renewcommand*{~}{\relax\ifmmode\sim\else\nobreakspace{}\fi}%GET TILDE FOR "IS DISTRIBUTED AS"
\newcommand{\Expect}{\mbox{{\normalfont E}}}
\newcommand{\Ex}{{\rm{I\hspace{-.75mm}E}}}
\newcommand{\se}{\mbox{s.e.}}
\newcommand{\sehat}{\widehat{\mbox{s.e.}}}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\Varhat}{\widehat{\mbox{Var}}}
\newcommand{\Cov}{\mbox{Cov}}
\newcommand{\Covhat}{\widehat{\mbox{Cov}}}
\newcommand{\Corr}{\mbox{Corr}}
\newcommand{\mse}{\mbox{mse}}
\newcommand{\PFS}{P\{\mbox{FS}\}}
\newcommand{\PFSi}{P\{\mbox{FS}_i\}}
\newcommand{\PCS}{P\{\mbox{CS}\}}

\newcommand{\evalat}{\biggl.\biggr|}

%parentheses
\newcommand{\lpr}{\left(}     \newcommand{\rpr}{\right)}
\newcommand{\lcbr}{\left\{}  \newcommand{\rcbr}{\right\}}
\newcommand{\lbr}{\left[}     \newcommand{\rbr}{\right]}
\newcommand{\ld}{\left.}      \newcommand{\rd}{\right.}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}

%mbox shortcuts
\newcommand{\myand}{\quad\mbox{and}\quad}
\newcommand{\myor}{\quad\mbox{or}\quad}
\newcommand{\myif}{\mbox{if }}
\newcommand{\myfor}{\mbox{for }}
\newcommand{\mywp}{\mbox{w.p. }}


%%% FORMATTING SHORTCUTS -----------------------------------------------------------------------------

\newcommand{\thme}[2]{{\begin{theorem}[#1]#2\end{theorem}}}
\newcommand{\prope}[2]{{\begin{proposition}[#1]#2\end{proposition}}}
\newcommand{\leme}[2]{{\begin{lemma}[#1]#2\end{lemma}}}
\newcommand{\core}[2]{{\begin{corollary}[#1]#2\end{corollary}}}
\newcommand{\resulte}[2]{{\begin{result}[#1]#2\end{result}}}
\newcommand{\assume}[2]{{\begin{assumption}[#1]#2\end{assumption}}}
\newcommand{\remarke}[2]{{\begin{remark}[#1]#2\end{remark}}}
\newcommand{\defne}[2]{\begin{definition}[#1]#2\end{definition}}
\newcommand{\exe}[2]{{\begin{example}[#1]#2\end{example}}}
\newcommand{\myproof}[2]{{\begin{proof}[#1]#2\end{proof}}}

\newenvironment{itemizec}
{ \begin{itemize}[nosep]    }
{ \end{itemize}                  } 

%%% LETTERS -----------------------------------------------------------------------------

%STATISTICAL LETTERS

%BARS -------------------------
%bars: roman
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
% \newcommand{\hbar}{\bar{h}}
%bars: greek
\newcommand{\Gammabar}{\bar{\Gamma}}
\newcommand{\Phibar}{\bar{\Phi}}

%HATS -------------------------
%hats: roman
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ellhat}{\hat{\ell}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\phat}{\hat{p}}
\newcommand{\shat}{\hat{s}}
\newcommand{\what}{\hat{w}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
%hats: greek
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\betahat}{\hat{\beta}}
\newcommand{\varepsilonhat}{\hat{\varepsilon}}
\newcommand{\lambdahat}{\hat{\lambda}}
\newcommand{\muhat}{\hat{\mu}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\Gammahat}{\widehat{\Gamma}}
\newcommand{\Sigmahat}{\widehat{\Sigma}}

%TILDE -------------------------
\newcommand{\gtilde}{\tilde{g}}
\newcommand{\ztilde}{\tilde{z}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Ftilde}{\widetilde{F}}
%tilde: greek
\newcommand{\alphatilde}{\tilde{\alpha}}
\newcommand{\Deltatilde}{\widetilde{\Delta}}
\newcommand{\deltatilde}{\tilde{\delta}}

%CHECK -------------------------
\newcommand{\Ncheck}{\check{N}}
\newcommand{\BFXcheck}{\check{\BFX}}


%BOLDFACE -- for compatibility with INFORMS formats
%roman LOWER
\newcommand{\BFa}{\bm{a}}
\newcommand{\BFb}{\bm{b}}
\newcommand{\BFc}{\bm{c}}
\newcommand{\BFd}{\bm{d}}
\newcommand{\BFe}{\bm{e}}
\newcommand{\BFf}{\bm{f}}
\newcommand{\BFg}{\bm{g}}
\newcommand{\BFh}{\bm{h}}
\newcommand{\BFp}{\bm{p}}
\newcommand{\BFs}{\bm{s}}
\newcommand{\BFt}{\bm{t}}
\newcommand{\BFu}{\bm{u}}
\newcommand{\BFw}{\bm{w}}
\newcommand{\BFx}{\bm{x}}
\newcommand{\BFy}{\bm{y}}
\newcommand{\BFz}{\bm{z}}
%roman UPPER
\newcommand{\BFE}{\bm{E}}
\newcommand{\BFF}{\bm{F}}
\newcommand{\BFG}{\bm{G}}
\newcommand{\BFH}{\bm{H}}
\newcommand{\BFP}{\bm{P}}
\newcommand{\BFW}{\bm{W}}
\newcommand{\BFU}{\bm{U}}
\newcommand{\BFX}{\bm{X}}
\newcommand{\BFS}{\bm{S}}
\newcommand{\BFY}{\bm{Y}}
\newcommand{\BFZ}{\bm{Z}}
%greek
\newcommand{\BFalpha}{\bm{\alpha}}
\newcommand{\BFbeta}{\bm{\beta}}
\newcommand{\BFdelta}{\bm{\delta}}
\newcommand{\BFDelta}{\bm{\Delta}}
\newcommand{\BFepsilon}{\bm{\epsilon}}
\newcommand{\BFvarepsilon}{{\bm{\varepsilon}}}
\newcommand{\BFtheta}{\bm{\theta}}
\newcommand{\BFphi}{\bm{\phi}}
\newcommand{\BFgamma}{\bm{\gamma}}
\newcommand{\BFlambda}{\bm{\lambda}}
\newcommand{\BFLambda}{\bm{\Lambda}}
\newcommand{\BFnu}{\bm{\nu}}
\newcommand{\BFmu}{\bm{\mu}}
\newcommand{\BFomega}{\bm{\omega}}
\newcommand{\BFOmega}{\bm{\Omega}}
\newcommand{\BFrho}{\bm{\rho}}
%symbols
\newcommand{\BFzero}{\bm{0}}
\newcommand{\BFinfty}{\bm{\infty}}


%TWO OR MORE MODIFICATIONS

%bold and bar: roman
\newcommand{\BFybar}{\bar{\BFy}}
\newcommand{\BFEbar}{\bar{\BFE}}
\newcommand{\BFFbar}{\bar{\BFF}}
\newcommand{\BFGbar}{\bar{\BFG}}
\newcommand{\BFXbar}{\bar{\BFX}}
\newcommand{\BFYbar}{\bar{\BFY}}

%bold and hat: roman
\newcommand{\BFGhat}{\hat{\BFG}}
\newcommand{\BFHhat}{\hat{\BFH}}
\newcommand{\BFXhat}{\hat{\BFX}}
\newcommand{\BFYhat}{\hat{\BFY}}
%bold and hat: greek
\newcommand{\BFalphahat}{\hat{\BFalpha}}
\newcommand{\BFvarepsilonhat}{\hat{\BFvarepsilon}}
\newcommand{\BFthetahat}{\hat{\BFtheta}}

%bold and tilde: roman
\newcommand{\BFxtilde}{\widetilde{\BFx}}
\newcommand{\BFXtilde}{\widetilde{\BFX}}
\newcommand{\BFytilde}{\widetilde{\BFy}}
\newcommand{\BFYtilde}{\widetilde{\BFY}}
%bold and tilde: greek
\newcommand{\BFalphatilde}{\tilde{\BFalpha}}


%bar and hat: greek
\newcommand{\sigmabarhat}{\hat{\bar{\sigma}}}

%MATHSF
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfz}{\mathsf{z}}

\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfZ}{\mathsf{Z}}



%MATHCAL 
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcJ}{\mathcal{J}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcS}{\mathcal{S}}
\newcommand{\mcs}{\mathcal{s}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcZ}{\mathcal{Z}}

%mathcal and bar
 \newcommand{\mcDbar}{\bar{\mcD}}
 \newcommand{\mcEbar}{\bar{\mcE}}
 \newcommand{\mcPbar}{\bar{\mcP}}
%mathcal and hat
\newcommand{\mcDhat}{\hat{\mcD}} 
\newcommand{\mcEhat}{\hat{\mcE}} 
\newcommand{\mcPhat}{\hat{\mcP}}
 \newcommand{\mcShat}{\hat{\mcS}}
 %mathcal and tilde
 \newcommand{\mcYtilde}{\widetilde{\mcY}}
\newcommand{\mcOtilde}{\widetilde{\mcO}}

%MATHBB 
\newcommand{\mbA}{\mathbb{A}}
\newcommand{\mbB}{\mathbb{B}}
\newcommand{\mbC}{\mathbb{C}}
\newcommand{\mbD}{\mathbb{D}}
\newcommand{\mbE}{\mathbb{E}}
\newcommand{\mbF}{\mathbb{F}}
\newcommand{\mbG}{\mathbb{G}}
\newcommand{\mbH}{\mathbb{H}}
\newcommand{\mbI}{\mathbb{I}}
\newcommand{\mbJ}{\mathbb{J}}
\newcommand{\mbK}{\mathbb{K}}
\newcommand{\mbL}{\mathbb{L}}
\newcommand{\mbM}{\mathbb{M}}
\newcommand{\mbN}{\mathbb{N}}
\newcommand{\mbO}{\mathbb{O}}
\newcommand{\mbP}{\mathbb{P}}
\newcommand{\mbQ}{\mathbb{Q}}
\newcommand{\mbR}{\mathbb{R}}
\newcommand{\mbS}{\mathbb{S}}
\newcommand{\mbT}{\mathbb{T}}
\newcommand{\mbU}{\mathbb{U}}
\newcommand{\mbV}{\mathbb{V}}
\newcommand{\mbW}{\mathbb{W}}
\newcommand{\mbX}{\mathbb{X}}
\newcommand{\mbY}{\mathbb{Y}}
\newcommand{\mbZ}{\mathbb{Z}}

%MATHFRAK
\newcommand{\mfz}{{\mathfrak{z}}}
\newcommand{\mfE}{\mathfrak{E}}
\newcommand{\mfS}{\mathfrak{S}}

%mathbb with hat
\newcommand{\mbEhat}{\hat{\mbE}}
\newcommand{\mbVhat}{\hat{\mbV}}

%%% SPACING -----------------------------------------------------------------------------

\newcommand{\spc}{\vspace{.15in}}
\newcommand{\fillpg}{\vspace*{\fill}}

%%% OPERATIONS -----------------------------------------------------------------------------

\newcommand{\defn}{\mathrel{\mathop:}=}
\newcommand{\nfed}{=\mathrel{\mathop:}}
\newcommand{\seteq}{\stackrel{\mbox{\footnotesize{set}}}{=}}


  
%%% TREATMENT OF FIGURES -----------------------------------------------------------------------------
    % Alter some LaTeX defaults for better treatment of figures:
    % See p.105 of "TeX Unbound" for suggested values.
    % See pp. 199-200 of Lamport's "LaTeX" book for details.
    %   General parameters, for ALL pages:
    \renewcommand{\topfraction}{0.9}	% max fraction of floats at top
    \renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{2}
    \setcounter{totalnumber}{4}     % 2 may work better
    \renewcommand{\textfraction}{0.05}	% allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
    \renewcommand{\floatpagefraction}{0.85}	% require fuller float pages
	% N.B.: floatpagefraction MUST be less than topfraction !!
    \renewcommand{\dblfloatpagefraction}{0.85}	% require fuller float pages

\pdfminorversion=6 

